Entanglement Diagnostics for Efficient Quantum Computation

We consider information spreading measures in randomly initialized variational quantum circuits and introduce entanglement diagnostics for efficient variational quantum/classical computations. We establish a robust connection between entanglement measures and optimization accuracy by solving two eigensolver problems for Ising Hamiltonians with nearest-neighbor and long-range spin interactions. As the circuit depth affects the average entanglement of random circuit states, the entanglement diagnostics can identify a high-performing depth range for optimization tasks encoded in local Hamiltonians. We argue, based on an eigensolver problem for the Sachdev-Ye-Kitaev model, that entanglement alone is insufficient as a diagnostic to the approximation of volume-law entangled target states and that a large number of circuit parameters is needed for such an optimization task.

==> others.tex <==

$c_{eff}$ can be understood as an effective thermal entropy density, which we can deduce
from the first law of thermodynamics:
 \begin{equation}
        c_{eff} = \frac{\Delta(\varepsilon)}{n_A  T_{eff}} \ ,
    \end{equation}
    where $\varepsilon$ is the energy density and
    \begin{equation}
        \Delta(\varepsilon) = \varepsilon(initial~ state) - \varepsilon(ground~ state) \ ,
    \end{equation}
is the energy density
    of the initial state relative to the ground state.
   
    
The correlation length of the system is:
\begin{equation}
    \xi \sim \frac{1}{T_{eff}} \ .
\end{equation}


On this subspace one finds a two-parameter family of symmetry charges:
\begin{equation}
 Q =
 \begin{pmatrix}
 q_1+q_2  & 0 & 0 & 0\\
 0 & q_1 & q_2  & 0 \\
 0 & q_2 & q_1  & 0 \\ 
  0 & 0 & 0  &  q_1+q_2 \\
\end{pmatrix}    
    \ .    
\end{equation}


\begin{equation}
P =     \begin{pmatrix}
1  & 0 \\
\\
0 & -1 
\end{pmatrix} \ ,
\end{equation}
\subsection{Complete Graph Conserved Charges}
Consider first the case $n=2$ qubits with $L$ layers.
The network operator reads:
\begin{equation}
O_{net} = \prod_{i=1}^L Z R(\theta_{2i})\otimes R(\theta_{1i}) \ ,    
\end{equation}
where
$Z=I\oplus P$ with $P$ the reflection
\begin{equation}
P =     \begin{pmatrix}
1  & 0 \\
\\
0 & -1 
\end{pmatrix} \ ,
\end{equation}
and $R(\theta)$ is a rotation around the $y$-axis
\begin{equation}
R(\theta) =     \begin{pmatrix}
Cos[\frac{\theta}{2}] & -Sin[\frac{\theta}{2}] \\
\\
Sin[\frac{\theta}{2}] & Cos[\frac{\theta}{2}] 
\end{pmatrix} \ .
\end{equation}
We look for integrable directions in the $2L$-dimensional
parameter space $(\theta_{11},\theta_{21},...,\theta_{1L},\theta_{2L})$ by searching for conserved charges.
For a classical system with $k$ degrees of freedom to be integrable one needs $k$ conserved charges in involution.

The charges should satisfy:
\begin{equation}
 \left[Q,O_{net}\right] = 0 \ . 
 \label{commute}
\end{equation}
One can solve (\ref{commute}) on the $n$-dimensional submanifold
$\theta_{2i}=0, i=1,...,L$ where:
\begin{equation}
R(\theta_{1i})\otimes R(\theta_{2i}) = R(\theta_{1i})\otimes I
,~~~~ i=1,...,L \ .
\end{equation}
and find a one parameter family of conserved charges:
\begin{equation}
    Q = \hat{q}\oplus\hat{q},~~~~
\hat{q} =
 \begin{pmatrix}
 1 & 0 \\
 0 & -1 \\
\end{pmatrix}    
    \ . 
\end{equation}

\begin{itemize}
    \item This calculation raises a question. If we started by
    not acting on the second qubit with the rotation
    gate around the $y$-axis, will we get a better convergense ?
It seems that this subspace is not good and there is no entanglement.    
\end{itemize}
Another solution is on the subspace 
$\theta_{1i} = \theta_{2i} = c_i, i=1,...,L$.
On this subspace one finds a two-parameter family of symmetry charges:
\begin{equation}
 Q =
 \begin{pmatrix}
 q_1+q_2  & 0 & 0 & 0\\
 0 & q_1 & q_2  & 0 \\
 0 & q_2 & q_1  & 0 \\ 
  0 & 0 & 0  &  q_1+q_2 \\
\end{pmatrix}    
    \ .    
\end{equation}
\begin{itemize}
    \item Is this the most general solution ? 
\end{itemize}




\begin{itemize}
    \item How do we know that the subspace $U(\theta)|0>$
    is close to the ground state of the Hamiltonian ?
    \item In order to characterize the spreading of an operator
    we can expand it in a basis of local operators
    \begin{equation}
 U^{\dagger}H U = \sum_{\alpha}C_{\alpha} O_{\alpha} \ ,       
    \end{equation}
  and calculate the entropy
  \begin{equation}
      S = -\sum_{\alpha}|C_{\alpha}|^2 Log |C_{\alpha}|^2 \ .
  \end{equation}
In fact we can ask more generally about the scaling with time 
of the Renyi entropy associated with the operator spread.
\item One can also inquire what is the relation between these
entropies  and the entanlgement entropies that have been generated
by the quantum gates.



We can try to check how much entanglement we generate in the circuit.
Suppose we have $n$ qubits and let's divide to two groups
$n_A,n_B, n_A \leq n_B, n_A+n_B=n$.
Let is calculate the reduced density matrix of our state
as a functiin of time:
\begin{equation}
\rho_A(t) = Tr_B \left(\rho(t)\right) \ .
    \end{equation}
Question: how does the purity 
\begin{equation}
    I(t) = Tr_A \left(\rho_A^2\right) \ ,
\end{equation}
decay with time.
If we average over the uniform distribution
it should probably decay exponentially.
What happens along the trajectory that we are following
trying to get to the minimum.

\item Do conserved charges limit the growth of entanglement ?

\end{itemize}


\begin{itemize}

\item We can change the architecture of the circuit - viewed as a graph we should not have a complete
graph but a much more sparse one, like an Expander graph.
This has two advantages: first, from theoretical point of view the more local ${U}^{\dagger}(\theta) H U$
the longer it takes for it to spread.
Second, a complete graph cannot be designed as a physical quantum circuit.
Can we identify better circuit architectures based on graph properties ?
If we are concerned with operator mixing then it seems that the right think to do is
to study random walk on a graph.

\item A possible direction to follow is to view the spread of the operator as a random motion and estimate the mean and the variance
of the spread. This depends on the circuit architecture.
We can analyze the functional relationship between the 
variance of the spread and the Hessian of the gradient motion in parameter space.
\item We can change the distribution from which we draw the parameters. Since the random quantum circuit is a graph, we
can think about a (biased) random motion on a graph.

\end{itemize}


We expect that the entanglement property of initial states should be sufficient to predict whether the optimization outcome will be good or bad. Let's pick some specific states with distinct optimization outcomes, and calculate their Renyi-2 entropies with different choices of subregions. 




\begin{itemize}
    \item Does the optimization respect the "foliation" structure by entanglement? 


When $p=\frac{1}{2}$ we should have zero $v_B$ and zero spread. Can we check that ?
Can we see what does it does it do for optimization ?
The other extreme limit is $v_B=1$, where there is a maximal spread.


\item It is possible that the complexity of the mixing caused by the diffusion is actually secondary to the more complex mixing of entanglement.
In particular, the scaling of the scrambling time due to diffusion is different 
than the one due to entanglement. That means that these two diagnostics of chaos
are very different on different graphs. More later.

\item In general, it would be interesting to quantify the difference in the operator
spreading between chaotic and integrable systems (there is already some work in this).

\item It seems that the only exponent in the problem is the
velocity $v_b$. Is it true the scaling of the entanglement entropy
is also determined by $v_b$?
This seems to be not the case and these are independent quantities.

\item The importance of the Hamiltonian: intuitively it is clear that the more local the Hamiltonian the less spread is expected.
We need to charaterize it.







\end{itemize}



For the entanglement entropy:
\begin{equation}
|S_A(\rho_{g}) - S_A(\rho_{c})|
\leq \Delta \log (2^{n_A}-1)- \Delta\log \Delta - (1-\Delta) \log (1-\Delta) \simeq 
n_A \Delta \ ,
\end{equation}
and the Renyi entropies:
\begin{equation}
|{\cal R}_A^k(\rho_{g}) - {\cal R}^k_A(\rho_{c})|
\leq \frac{2^{n_A(k-1)}}{k-1}\left(1 - (1-\Delta)^k - (2^{n_A}-1)^{k-1} \Delta^k \right) 
\simeq \frac{k \Delta 2^{n_A(k-1)}}{k-1} \ 
\end{equation}
where the approximation is for $\Delta\ll 1$.


\section{Opreator Spreading}

Operator spreading is another diagnostic of the chaotic dynamics and information scrambling. A local operator $\mathcal{O}$ that acts on a small number of qubits at time
step $t=0$ evolves at time step $t$ to
\begin{equation}
\mathcal{O}(t) = U(t)^{\dagger} \mathcal{O}(0) U(t)
\label{evo}
\end{equation}
that acts on a large number of qubits.
This spread can be quantified and its growth is ballistic with a characteristic velocity
called the butterfly velocity.
In our case, the value of the butterfly velocity depends on the circuits architecures
and the type of its quantum gates.
In this section we will study this diagnostic and discuss the relationship and differences
from the entanglement diagnostic.

\subsection{Butterfly Velocity} 
Any Hermitian operator $\mathcal{O}(t)$ acting on $n$ qubit systems can be written in the Pauli string basis: 
\begin{align}
    \mathcal{O}(t) = \frac{1}{2^{n/2}}\sum_{j_1, \cdots, j_n} h_{j_1,\cdots,j_n}(t)\,  \sigma_{j_1}^{(1)}\otimes \cdots \otimes \sigma_{j_n}^{(n)} \ ,
\end{align}
where 
\begin{align}
    h_{j_1,\cdots,j_n}(t) \equiv\frac{1}{2^{n/2}} \text{Tr}(\sigma_{j_1}^{(1)}\otimes \cdots \otimes \sigma_{j_n}^{(n)}  \cdot \mathcal{O}(t)) \ .
\end{align}
Under the unitary time evolution (\ref{evo})
\begin{align}
    \text{Tr}(\mathcal{O}(t)^\dagger \mathcal{O}(t))  = \text{Tr}(\mathcal{O}(0)^\dagger \mathcal{O}(0)) = \frac{1}{2^n}\sum \vert h_{j_1,\cdots,j_n}(t)\vert^2 = \text{constant} \ .
\end{align}

The size of the operator $\mathcal{O}(t)$ is measured by the size of the region where $\mathcal{O}(t)$ does not commute with
a typical local operator $\sigma_a^{(x)}$ at position $x$, which can be quantified as
\begin{align}
\mathcal{C}(x, t) &= \frac{1}{2}\text{Tr} (\rho_\infty [\mathcal{O}(t), \sigma_a^{(x)}]^\dagger [\mathcal{O}(t), \sigma_a^{(x)}])  = \frac{1}{2}\text{Tr} ( [\mathcal{O}(t), \sigma_a^{(x)}]^\dagger [\mathcal{O}(t), \sigma_a^{(x)}]) \nonumber \\
&= \sum_{\substack{j_1,\cdots,j_n \\j_x \neq 0, a}} 2 \vert h_{j_1,\cdots,j_n}(t)\vert^2
\label{c}
\end{align}
We would like to measure (\ref{c}) where the operator ${\cal O}(0)$ is the
Hamiltonian whose expectation value we are minimizing.



It has been argued that the operator spreading in the random quantum circuit
follows 
a one-dimensional biased random walk with probability $p$ of shrinking 
and $1-p$ for expanding \cite{Nahum:2017yvy}.
The mean of the spread reads:
\begin{equation}
\mu = (1-2p)t = v_B t \ ,
\label{\mu}
\end{equation}
where $t$ is the time (number of a gates), $v_B$ is the butterfly velocity $0 \leq v_B \leq 1$
and the variance 
\begin{equation}
\sigma = \left(2p(1-p)t\right)^{\frac{1}{2}} =
\left((1-v_B^2)t\right)^{\frac{1}{2}} \ .
\end{equation}
Using $p=\frac{1}{5}$ for generic four by four unitary matrices (the two-qubit gates), one evaluates the mean and variance
which are consistent with Figure *. We see
that the operator spread growth follows the same pattern as the entropy diagnostics but reaches
the plateau faster. This can be different for other graph architectures.
The value of $p$ depends on the circuit architecture and we can change it by a biased selection of matrices, hence changing the butterfly velocity.

\subsection{Numerical Simulation}




\section{Conserved Charges}

Conserved charges can slow down the process of information scrambling
and entanglement.
They can slow the ballistic growth of operator spreading \cite{sub}.
We will see that while the use of conserved charges allows for an efficient optimization, one has the risk that the ground state of the Hamiltonian
is not and eigenstate of the conserved charge in which case we are limited
by how close we can get to it.


\subsection{Random Quantum Circuit Conserved Charges}

The basic 2-qubit gate ${\cal O}_2$ that we use in the circuit is depicted in figure 1b. The operator reads:
\begin{equation}
{\cal O}_2 = Z R(\theta_{l,i})\otimes R(\theta_{l,j}) \ ,    
\end{equation}
where
$Z=diag[1,1,1-1]$
and $R(\theta)$ is a rotation around the $y$-axis.
It is straightforward to see that $[{\cal O}_2,Q]$ on the subspace
$\theta_{l,i} = \theta_{l,j}$ with $Q$ being 
a two-parameter family:
\begin{equation}
 Q =
 \begin{pmatrix}
 q_1+q_2  & 0 & 0 & 0\\
 0 & q_1 & q_2  & 0 \\
 0 & q_2 & q_1  & 0 \\ 
  0 & 0 & 0  &  q_1+q_2 \\
\end{pmatrix}    
    \ .    
\end{equation}
In general, $Q$ are symmetry charges on the subspace:
\begin{equation}
\theta_{1i} = \theta_{2i} = c_i, i=1,...,L \ .
\label{sub}
\end{equation}
We would like to see the effect of constraining to the subspace 
(\ref{sub}) on the growth of the entanglement entropy and
on the efficiency and success of the optimization.
Note, that the symmetry charges have a similar effect also on the operator spreading growth.


\subsection{Numerical Simulation}

{\color{red} We need the growth of the entanglement entropy and the form of the optimization}.




\section{Spectral Form Factor}

The spectral for factor of the eigenvalue spectrum of the reduced density 
$\rho_A$ can be used as a diagnostic of quantum chaos. In this section we will use 
it as yet another characteristic of region $A$.
{\color{red} Does the Ising ground state exhibits a "ramp" ?
Can this be a distinguishing feature from the SYK}

Define:
\begin{equation}
Z(\tau) = Tr e^{-i \tau \rho_A} \ ,    
\end{equation}
where $\rho_A$ is the reduced density matrix of the circuit. The dimension
of the Hilbert space is $dim H = Z(0) = N$ and $\rho_A$ is an $N\times N$ matrix. 
Define:
\begin{equation}
 g(\tau) = \langle Z(\tau \bar{Z(\tau)} \rangle  \ .   
\end{equation}
$g(\tau)$ exhibits a ramp-like behaviour and it serves as a diagnostic
of quantum chaos.
We will be interested in $\frac{|Z(\tau)|^2}{Z(0)^2}$.

Consider first the case that $\rho$ is a reduced density matrix
of a product state and hence a pure state.
In this case:
\begin{equation}
Z(\tau) = \frac{(N-1) + e^{-i \tau }}{N},~~~|Z(\tau)|^2 = N -2 + \frac{2}{N} + \frac{2(N-1)}{N^2} Cos(\tau) \ .    
\end{equation}
Consider next the completely mixed state $\rho = \frac{I}{N}$.
\begin{equation}
Z(\tau) = N e^{-i \frac{\tau}{N} },~~~|Z(\tau)|^2 = N^2 \ .    
\end{equation}
Consider the thermal distribution:
$\rho= diag[\lambda_1,...,\lambda_N]$
where  $\lambda_k= \frac{e^{-\beta E_k}}{\sum_i e^{-\beta E_i}}$ \ .
In this case:
\begin{equation}
|Z(\tau)|^2 = N +   \sum_{i\neq j}^N Cos(\frac{(\lambda_i-\lambda_j)\tau}{N}) \leq N^2 \ ,
\end{equation}
where equality is when $\beta=0$.
Thus, in the range between the non-mixed and fully mixed density matrices
we have at large $N$:
\begin{equation}
  \frac{1}{N} \leq \frac{|Z(\tau)|^2}{Z(0)^2} \leq 1 \ .
\end{equation}

{\color{red} Can we plot spectral form factor for the circuit ?}

\begin{figure}
\centering
\includegraphics[height=6cm]{figs/SFFQ12.pdf}
\includegraphics[height=6cm]{figs/SFFQ14.pdf}
\caption{(a) The averaged spectral form factor ${|Z(\tau)|^2}/{Z(0)^2}$ at $N=12$. (b) The averaged spectral form factor ${|Z(\tau)|^2}/{Z(0)^2}$ at $N=14$}
\label{fig:SFF}
\end{figure}


\subsection{Complete Graph}

The circuit is depicted in figure *.
The plot of entanglement as a function of the number of layers is 
given in figure *.
We see that in this case the fact that all the qubits are linked to each other
already in the first layer implies that the entanglement reaches saturation
by a very shallow circuit, i.e. effective one layer {\color{red} True ?}


\bibitem{bound}
Chen, Z., Ma, Z., Nikoufar, I. et al. Sharp continuity bounds for entropy and conditional entropy. Sci. China Phys. Mech. Astron. {\bf 60}, 020321 (2017). 
https://doi.org/10.1007/s11433-016-0367-x


\begin{figure}[H]
\centering
    \includegraphics[width=\textwidth]{figs/optim-Q8-SYK2.pdf}
    \caption{The optimization to reach the ground state of the SYK model for different numbers of circuit layers with $n=8$ qubits.
    Left: The difference between the circuit state and the ground state energy as a function of the number of optimization steps. Middle: The trace distance between circuit state and the ground state as a function of the number of optimization steps. Right: The difference between the circuit state and the ground state Renyi entropies
    as a function of the number of optimization steps. All the three diagnsotics show that optimization does not work.}
\end{figure}




\appendix
\section{Circuit Conserved Charges and Restricted Parametrization}

The basic 2-qubit gate ${\cal O}_2$ that we used in the random 
quantum reads:
\begin{equation}
{\cal O}_2 = Z R(\theta_{l,i})\otimes R(\theta_{l,j}) \ ,    
\end{equation}
where
$Z=diag[1,1,1-1]$
and $R(\theta)$ is a rotation around the $y$-axis.
It is straightforward to see that $[{\cal O}_2,Q]$ on the subspace
$\theta_{l,i} = \theta_{l,j}$ with $Q$ being 
a two-parameter family:
\begin{equation}
 Q =
 \begin{pmatrix}
 q_1+q_2  & 0 & 0 & 0\\
 0 & q_1 & q_2  & 0 \\
 0 & q_2 & q_1  & 0 \\ 
  0 & 0 & 0  &  q_1+q_2 \\
\end{pmatrix}    
    \ .    
\end{equation}
In general, $Q$ are symmetry charges on the subspace:
\begin{equation}
\theta_{1i} = \theta_{2i} = c_i, i=1,...,L \ .
\label{sub}
\end{equation}
We would like to see the effect of constraining to the subspace 
(\ref{sub}) on the growth of the entanglement entropy and
on the efficiency and success of the optimization.

\subsection{Entanglement Diagnostics}

\begin{figure}[H]
\centering
\includegraphics[height=5.8cm]{figs/entropygrowth - LayerEqual.pdf}
\caption{Von Neumann and Renyi-2 entropies averaged over 50 random circuits, whose circuit parameters at an individual layer are equal and randomly drawn from the uniform distribution $\mathcal{U}(0, 2\pi)$ as a function of the number of layers. }
\label{fig:entropy-growth-layerequal}
\end{figure}

\begin{figure}[H]
\centering
    \includegraphics[height=5.8cm]{figs/entropies - LayerEqual.pdf} 
\caption{Various entanglement entropies averaged over $50$ random circuits, whose circuit parameters at an individual layer are equal and randomly drawn from the uniform distribution $\mathcal{U}(0, 2\pi)$ as a function of the number of layers. }
\label{fig:entropies-layerequal}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[height=5.8cm]{figs/entropy - min-max - LayerEqual.pdf}
    \caption{The sample mean of $S_\text{max}$, $S_\text{min}$, $S_\text{max}- S_\text{min}$ over $50$ instances of random circuits, whose circuit parameters at an individual layer are equal and randomly drawn from the uniform distribution $\mathcal{U}(0, 2\pi)$ }
    \label{fig:my_label}
\end{figure}


\begin{figure}[H]
\centering
\includegraphics[height=5.8cm]{figs/geometry - LayerEqual.pdf}
\caption{The Geometric measure 
of entanglement (\ref{geometric}) averaged over 50 random circuits, whose circuit parameters at an individual layer are equal and randomly drawn from the uniform distribution $\mathcal{U}(0, 2\pi)$ as a function of the number of layers. }
\label{fig:geometry-layerequal}
\end{figure}




\begin{figure}[H]
\centering
\includegraphics[height=5.8cm]{figs/inequality - LayerEqual.pdf}
\caption{Inequality (2.12) at $n=12$ qubits, averaged over $50$ random circuits, whose circuit parameters at an individual layer are equal and randomly drawn from the uniform distribution $\mathcal{U}(0, 2\pi)$ }
\label{fig:inequality-layerequal}
\end{figure}

\subsection{Optimization}


==> preamble.tex <==
%--------------
%% preamble.tex
%% this should be included with a command like
%% \input{preamble.tex}


%\documentclass[12pt]{article}
\usepackage[utf8]{inputenc}
%\usepackage{draftcopy}
%\usepackage{draftwatermark}

%%%%%%% Muli commands %%%%

\usepackage{color}
\usepackage{graphicx}
\graphicspath{ {./Images/} }
\usepackage{wrapfig}
%\usepackage{fullpage}
\usepackage{amsmath, amsthm, amssymb}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     filecolor=magenta,      
%     urlcolor=cyan,
% }
% \urlstyle{same}

\usepackage{theoremref}

%\newcommand\comment[1]{\fbox{\tt #1}}

%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}
%\renewcommand{\algorithmicrepeat}{}
%\renewcommand{\algorithmicuntil}{}
%\renewcommand{\algorithmicif}{\textbf{If}}
%\renewcommand{\algorithmicelse}{\textbf{Else }}
%\renewcommand{\algorithmicloop}{}
%\renewcommand{\algorithmicfor}{\textbf{For}}

\newtheorem{theorem}{Theorem}[section]
   \newtheorem{thm}{Theorem}[section]
   \newtheorem{conj}[thm]{Conjecture}
   \newtheorem{lemma}[thm]{Lemma}
   \newtheorem{corollary}[thm]{Corollary}
   \newtheorem{claim}[thm]{Claim}
   \newtheorem{proposition}[thm]{Proposition}
   \newtheorem{definition}{Definition}
   \newtheorem{remark}{Remark}
    \newtheorem{fact}{Fact}
    \newtheorem{assumption}{Assumption}
    \newtheorem{observation}{Observation}


\newcommand\subspaces[2] { \genfrac[]{0pt}{}{#1}{#2} }

\newcommand\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\Z{\mathbb{Z}}

\newcommand\card[1]{\left| {#1} \right|}

\newcommand\tup[1]{\left\langle #1 \right\rangle}

\newcommand\set[1]{{\left\{ #1 \right\}}}
\newcommand\Set[2]{ \left\{ #1 \vert #2\right\} }
\newcommand\sett[2]{\left\{ \left. #1 \;\right\vert #2 \right\}}
\newcommand\settright[2]{\left\{ #1 \;\left\vert\; #2 \right.\right\}}

\newcommand\Prob[2]{{\Pr_{#1}\left[ {#2} \right]}}
\newcommand\cProb[3]{{\Pr_{#1}\left[ \left. #3 \;\right\vert #2 \right]}}
\newcommand\cProbright[3]{{\Pr_{#1}\left[ #3\;\left\vert  #2\right. \right]}}
\newcommand\Expect[2]{{\mathop{\mathbb{E}}_{#1}\left[ {#2} \right]}}
\newcommand\cExpect[3]{{\mathop\mathbb{E}_{#1}\left[ \left. #3 \;\right\vert #2 \right]}}

\newcommand\ang[1]{\langle {#1}\rangle}

\newcommand\norm[1]{\| #1 \|}

\newcommand\power[1]{\set{0,1}^{#1}}

\newcommand\ceil[1]{\lceil{#1}\rceil}

\newcommand\round[1]{\left\lfloor{#1}\right\rfloor}

\newcommand\half{{1\over2}}
\newcommand\quarter{{1\over4}}
\newcommand\eigth{{1\over8}}

\newcommand\defeq{\stackrel{def}{=}}

\newcommand\skipi{{\vskip 10pt}}

\newcommand\IP[2]{\left\langle {#1}, {#2} \right\rangle}
\newcommand\inner[2]{\left\langle{#1},{#2}\right\rangle}

\newcommand\TF{ {\set{T, F}} }
\newcommand\pmo{ { \{\pm 1\} } }
\newcommand\Gn{ {\pmo^n} }
\newcommand\BF{ {\colon\Gn\to\pmo } }
\newcommand\cube[1]{ { \set{-1,1}^{#1} } }

\newcommand\nV{{\cal \#V}}
\newcommand\pV{{ p{\cal V} }}
\newcommand\tV{ {\cal \widetilde{V} } }

\newcommand\sqrtn{ {\sqrt n} }
\newcommand\eps{\epsilon}

\newcommand\minimum[2] {  \min\left\{{{#1}, {#2}}\right\}   }

\newcommand\spn{span}
\newcommand\spnn[1]{span({#1})}

\newcommand\Ext{{\sf s-Ext}}

\newcommand\Extt{{\sf Ext}}

\newcommand\sgn[1]{sign({#1})}

\newcommand*\xor{\mathbin{\oplus}}

\newcommand*\bxor{\mathbin{\bigoplus}}

\newcommand*\Hell[2]{{H\left({#1}, \ {#2}\right)}}

\newcommand*\cHell[4]{{H\left({#1}\vert({#2}),\ {#3}\vert({#4}) \right)}}

\newcommand*\QED{}

\newcommand*\Uni{{\cal U}}

%%%%%%% \end{Muli commands} %%%%
%%%%%%% \begin{Esty commands} %%%%
   \newtheorem{untruth}[thm]{Untruth}

\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}

\newcommand*\entropy{ {\cal H} }

\newcommand\parentheses[1]{{\left({#1}\right)}}
\newcommand\ps[1]{\parentheses{#1}}

\newcommand\brackets[1]{{\left[{#1}\right]}}
\newcommand\fcoefficient[2]{{\widehat{#1}\parentheses{#2}}}

\newcommand\sqfcoefficient[2]{{\widehat{#1}^2\parentheses{#2}}}

\newcommand\fchar[1]{{\chi_{#1}}}


\newcommand\pentropy[1]{{\entropy\brackets{#1}}}
\newcommand\hentropy[1]{\entropy_\half\brackets{#1}}
\newcommand\parentropy[1]{\entropy_p\brackets{#1}}
%charcters entropy
\newcommand\charentropy[1]{{\pentropy{\widehat{#1}^2}}}
\newcommand\charhentropy[1]{{\hentropy{\widehat{#1}^2}}}
%values entropy
\newcommand\valentropy[1]{{\pentropy{{#1}^2}}}

\newcommand\plog[1]{{\log\parentheses{#1}}}
\newcommand\pln[1]{{\ln\parentheses{#1}}}
\newcommand\pfrac[2]{{\parentheses{\frac{#1}{#2}}}}

% Symmetric difference of sets%
\newcommand\symdif{\vartriangle}

%function degree%
\newcommand\fdeg[1]{{deg\parentheses{#1}}}

%absolute value%
\newcommand\abs[1]{{\left\lvert{#1}\right\rvert}}


%TODO list%
\usepackage{soul}
\usepackage{xcolor}
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\technical[1]{\textcolor{gray}{#1}}
\newcommand\purple[1]{\textcolor{purple}{#1}}
\newcommand\yellow[1]{\textcolor{yellow}{#1}}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\assume[1]{\textcolor{orange}{#1}}

%some macroes%
%alpha fraction for: %
\newcommand\idxalpha[2]{{\alpha_{#2}}}
%derivative%
\newcommand\fInduct[2]{f_{{#1}({#2})}}
\newcommand\fD[1]{\fInduct{D}{#1}}
\newcommand\fDj{\fD{j}}
\newcommand\fA[1]{\fInduct{A}{#1}}
\newcommand\fAj{\fA{j}}
\newcommand\alphaD[1]{{\alpha_{#1}}}
\newcommand\alphaDj{\alphaD{j}}
\newcommand\fIndcutUpper[2]{f^{{#1}({#2})}}
\newcommand\fsigmaj{\fIndcutUpper{\sigma}{j}}
\newcommand\fpmsi[3]{{#1}^{{#2}({#3})}}
\newcommand\fpi[2]{\fpmsi{#1}{+}{#2}}
\newcommand\fmi[2]{\fpmsi{#1}{-}{#2}}
\newcommand\fsi[2]{\fpmsi{#1}{\sigma}{#2}}
\newcommand\fpj[1]{\fpi{#1}{j}}
\newcommand\fmj[1]{\fmi{#1}{j}}
\newcommand\fsj[1]{\fsi{#1}{j}}
\newcommand\fplus[1]{f^{+({#1})}}
\newcommand\fminus[1]{f^{-({#1})}}
\newcommand\fminusj{\fminus{j}}
\newcommand\fplusj{\fplus{j}}
\newcommand\betaj{\beta_j}
\newcommand\deltaj{\delta_j}
\newcommand\M[1]{{M\brackets{#1}}}
\newcommand\p[1]{{p\brackets{#1}}}
\newcommand\dkl[2]{D_{KL}\brackets{{#1},{#2}}}
\newcommand\dfu[1]{\dkl{#1}{U_{2^n}}}
\newcommand\SD[2]{SD\brackets{{#1},{#2}}}
\newcommand\pnorm[1]{{\norm{{#1}}_\p{{#1}}}}
\newcommand\gparam[1]{{\gamma\brackets{{#1}}}}
\newcommand\gpparam[2]{{\gamma_{#1}\brackets{{#2}}}}
\newcommand\noisyf[2]{T_{#1}[{#2}]}
\newcommand\frho{T_\rho[f]}

\newcommand\fDi{\partial_if}
%\renewcommand\betaj{{\frac{\half\norm{\fminusj}_2^2}{\norm{f}_2^2}}}
\newcommand\oneminusbetaj{{\frac{\half\norm{\fplusj}_2^2}{\norm{f}_2^2}}}
%\renewcommand\alphaDj{{\frac{\norm{\fDj}_2^2}{\norm{f}_2^2}}}

\renewcommand\fDj{\partial_jf}

\renewcommand\fminusj{{f^-}}
\renewcommand\fplusj{{f^+}}
%average%



%moments%
%second moment%
\newcommand\secmoment[2]{\Expc{{#2}\sim\Lambda {#1}}{|{#2}|^2}}
%first moment%
\newcommand\firstmoment[2]{\Expc{{#2}\sim\Lambda {#1}}{|{#2}|}}

%norms%
\newcommand\snorm[2]{\brokenvert\brokenvert{#2}\brokenvert\brokenvert_{#1}}
\newcommand\enorm[2]{\norm{#2}_{#1}}

%\usepackage{wasysym}
%\usepackage{comment}
%\usepackage{marvosym}
%\usepackage{bbold}
%\usepackage{breqn}



%log of norm relations
\newcommand\logparama[2]{{\log\frac{\norm{#2}_2}{\norm{#2}_{#1}}}}
\newcommand\logparam[1]{{\log\frac{\norm{#1}_2}{\norm{#1}_1}}}
\newcommand\logparamp[1]{\logparama{p}{#1}}


\newcommand\indicator[1]{{\mathbb 1}_{#1}}
%%%%%%% \end{Esty commands} %%%%

